Learning Object-Centered Autotelic Behaviors with Graph Neural Networks

Although humans live in an open-ended world and endlessly face new challenges, they do not have to learn from scratch each time they face the next one. Rather, they have access to a handful of previously learned skills, which they rapidly adapt to new situations. In artificial intelligence, autotelic agents, which are intrinsically motivated to represent and set their own goals, exhibit promising skill adaptation capabilities. However, these capabilities are highly constrained by their policy and goal space representations. In this paper, we propose to investigate the impact of these representations on the learning and transfer capabilities of autotelic agents. We study different implementations of autotelic agents using four types of Graph Neural Networks policy representations and two types of goal spaces, either geometric or predicate-based. By testing agents on unseen goals, we show that combining object-centered architectures that are expressive enough with semantic relational goals helps learning to reach more difficult goals. We also release our graph-based implementations to encourage further research in this direction.

==> CoLLAs 2022 Autotelic GNNs/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

% \newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> CoLLAs 2022 Autotelic GNNs/preamble.tex <==
\usepackage{hyperref}
\usepackage{ucs}
\usepackage{comment}
\usepackage{amsmath}
\usepackage{bbold}
%\usepackage{fancybox}%fait des boites
\usepackage{pbox}%fait des boites
\usepackage{tcolorbox}
\usepackage[font=small]{caption}
\usepackage{capt-of}
%\usepackage{subcaption} % incompatible with subfig
%\usepackage[numbers]{natbib}
\usepackage{bm}
\usepackage{graphicx}
\usepackage{cancel}
\usepackage{array}
\usepackage{multirow}
\usepackage{colortbl}
\usepackage{tikz}
\usepackage{xspace}
\usepackage{subfig}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage{soul}
\usepackage{enumitem}
\usepackage{comment}

%\usepackage{apalike}
%\usepackage{cite}

%\renewcommand{\cite}{\citep}

\newcommand{\dhh}{\mymath{dh}}
\newcommand{\vth}{\mymath{\vec \theta}}
\newcommand{\vthp}{\mymath{\vec \vth^\prime}}
\newcommand{\delth}{\mymath{\delta \vth}}
\newcommand{\delthp}{\mymath{\delta \vthp}}
\newcommand{\hth}{\mymath{h_{\vth}}}
\newcommand{\hdth}{\mymath{h_{\vth + \delth}}}
\newcommand{\grad}{\mymath{\nabla_{\vth}}}
\newcommand{\natgrad}{\mymath{\nabla^{nat}_{\vth}}}
\newcommand{\Mnat}{\mymath{\vec M_{\text{nat}}(\vth)}}
\newcommand{\Hess}{\mymath{\vec H(\vth)}}
\newcommand{\C}{\mymath{\bf C(\vth)}}
\newcommand{\kfac}{{\sc kfac}\xspace}
\newcommand{\cemrl}{{\sc cem-rl}\xspace}
\newcommand{\cemddpg}{{\sc cem-ddpg}\xspace}
\newcommand{\cemtdd}{{\sc cem-td3}\xspace}
\newcommand{\relu}{{\sc relu}\xspace}
\newcommand{\evorl}{{\sc erl}\xspace}
\newcommand{\hc}{{\sc half-cheetah-v2}\xspace}
\newcommand{\hop}{{\sc hopper-v2}\xspace}
\newcommand{\sw}{{\sc swimmer-v2}\xspace}
\newcommand{\ant}{{\sc ant-v2}\xspace}
\newcommand{\walk}{{\sc walker2d-v2}\xspace}
\newcommand{\muj}{{\sc mujoco}\xspace}
\newcommand{\geppg}{{\sc gep-pg}\xspace}
\newcommand{\pytorch}{{\sc PyTorch}\xspace}

\newcommand{\mdp}{{\sc mdp}\xspace}
\newcommand{\gamer}{{\sc gamer}\xspace}
\newcommand{\gargaml}{{\sc gargaml}\xspace}
\newcommand{\tddd}{{\sc td3}\xspace}

\newcommand{\gnn}{{\sc gnn}\xspace}
\newcommand{\mpgnn}{{\sc mpgnn}\xspace}
\newcommand{\mpgnns}{{\sc mpgnn}s\xspace}
\newcommand{\gnns}{{\sc gnn}s\xspace}
\newcommand{\cnn}{{\sc cnn}\xspace}
\newcommand{\cnns}{{\sc cnn}s\xspace}
\newcommand{\gorl}{{\sc gorl}\xspace}
\newcommand{\imrl}{{\sc imrl}\xspace}
\newcommand{\nl}{{\sc nl}\xspace}

%%% Math commands
\def\bbbr{{\rm I\!R}}
\def\bbbe{{\rm I\!E}}
\newcommand{\Esp}{{\bbbe}{}}
\renewcommand\Pr{P} % probability
\newcommand\esper[2]{\underset{#1}{\mathbb{E}} \left[#2\right]} % expectation
\newcommand\espernosubstack[2]{\mathbb{E}_{#1} \left[#2\right]} % expectation, without substacking #1
\newcommand\espernobr[1]{\underset{#1}{\mathbb{E}}} % expectation, without brackets
\newcommand\mymax[2]{\textmd{max}_{#1} ~ #2} % max
\newcommand\trace{\textmd{Tr}} % trace operator
\newcommand\erf{\textmd{erf}} % error function
\newcommand\diag{\textmd{diag}} % diagonal matrix
\newcommand\asinh{\textmd{asinh}} % arcsinh
\newcommand\Id{\mat{I}}% identity matrix
\newcommand{\rbd}{{\sc rbd}\xspace}
\newcommand{\rbfn}{{\sc rbfn}\xspace}
\newcommand{\rbfns}{{\sc rbfn}s\xspace}
\newcommand{\vips}{{\sc vips}\xspace}
\newcommand{\reps}{{\sc reps}\xspace}
\newcommand{\creps}{{\sc creps}\xspace}
\newcommand{\hireps}{{\sc hireps}\xspace}
\newcommand{\aaac}{{\sc a3c}\xspace}
\newcommand{\offpac}{{\sc offpac}\xspace}
\newcommand{\reinforce}{{\sc reinforce}\xspace}
\newcommand{\retrace}{{\sc retrace}\xspace}
\newcommand{\blackdrops}{{\sc black-DROPS}\xspace}
\newcommand{\rock}{{\sc rock}$^*$\xspace}
\newcommand{\ddpg}{{\sc ddpg}\xspace}
\newcommand{\naf}{{\sc naf}\xspace}
\newcommand{\qprop}{{\sc Q-prop}\xspace}
\newcommand{\acer}{{\sc acer}\xspace}
\newcommand{\pgql}{{\sc pgql}\xspace}
\newcommand{\ipg}{{\sc ipg}\xspace}
\newcommand{\cmaes}{{\sc cma-es}\xspace}
\newcommand{\cma}{{\sc cma}\xspace}
\newcommand{\nes}{{\sc nes}\xspace}
\newcommand{\xnes}{x{\sc nes}\xspace}
\newcommand{\pepg}{{\sc pepg}\xspace}
\newcommand{\rwr}{{\sc rwr}\xspace}
\newcommand{\crkr}{{\sc crkr}\xspace}
\newcommand{\gpomdp}{{\sc g(po)mdp}\xspace}
\newcommand\cems{\textsc{cem}s\xspace}
\newcommand\cem{\textsc{cem}\xspace}
\newcommand{\trpo}{{\sc trpo}\xspace}
\newcommand{\ppo}{{\sc ppo}\xspace}
\newcommand{\gps}{{\sc gps}\xspace}
\newcommand{\nac}{{\sc nac}\xspace}
\newcommand{\enac}{e{\sc nac}\xspace}
\newcommand{\inac}{i{\sc nac}\xspace}
\newcommand{\sac}{{\sc sac}\xspace}
\newcommand{\acktr}{{\sc acktr}\xspace}
\newcommand{\ilqg}{i{\sc lqg}\xspace}
\newcommand{\svg}{{\sc svg}\xspace}
\newcommand{\power}{{\sc PoWER}\xspace}
\newcommand{\pilco}{{\sc pilco}\xspace}
\newcommand{\PIBB}{{\sc pi$^{\mbox{\tiny BB}}$}\xspace}
\newcommand{\picma}{{\sc pi$^2$-cma}\xspace}
\newcommand{\pis}{{\sc pi$^{2}$}\xspace}
\newcommand{\ann}{{\sc ann}\xspace}
\newcommand{\anns}{{\sc ann}s\xspace}
\newcommand{\mlps}{{\sc mlp}s\xspace}
\newcommand{\mlp}{{\sc mlp}\xspace}
\newcommand{\rbf}{{\sc rbf}\xspace}
\newcommand{\lwpr}{{\sc lwpr}\xspace}
\newcommand{\nipals}{{\sc nipals}\xspace}
\newcommand{\cad}{{\sc cad}\xspace}
\newcommand{\lcs}{{\sc lcs}\xspace}
\newcommand{\lcss}{{\sc lcs}s\xspace}
\newcommand{\xcsf}{{\sc xcsf}\xspace}
\newcommand{\QR}{{\sc qr}\xspace}
\newcommand{\RR}{{\sc rr}\xspace}
\newcommand{\xcs}{{\sc xcs}\xspace}
\newcommand{\moe}{{\sc m}o{\sc e}\xspace}
\newcommand{\gmr}{{\sc gmr}\xspace}
\newcommand{\gmm}{{\sc gmm}\xspace}
\newcommand{\gmms}{{\sc gmm}s\xspace}
\newcommand{\dmps}{{\sc dmp}s\xspace}
\newcommand{\mdps}{MDPs\xspace}
\newcommand{\ilogmr}{{\sc ilo-gmr}\xspace}
\newcommand{\kdtrees}{{\em kd-trees}\xspace}
\newcommand{\libsvm}{{\sc libsvm}\xspace}
\newcommand{\svd}{{\sc svd}\xspace}
\newcommand{\rmrc}{{\sc rmrc}\xspace}
\newcommand{\nmse}{{\sc nmse}\xspace}
\newcommand{\nmae}{{\sc nmae}\xspace}
\newcommand{\imlm}{{\sc imlm}\xspace}
\newcommand{\mae}{{\sc mae}\xspace}
\newcommand{\ga}{{\sc ga}\xspace}
\newcommand{\pls}{{\sc pls}\xspace}
\newcommand{\ls}{{\sc ls}\xspace}
\newcommand{\sr}{{\sc SR}\xspace}
\newcommand{\rlearning}{RL\xspace}
\newcommand{\drl}{deep RL\xspace}
\newcommand{\Drl}{Deep RL\xspace}
\newcommand{\dqn}{{\sc dqn}\xspace}
\newcommand{\rls}{{\sc rls}\xspace}
\newcommand{\krls}{{\sc krls}\xspace}
\newcommand{\rfrls}{{\sc rfrls}\xspace}
\newcommand{\irfrls}{i{\sc rfrls}\xspace}
\newcommand{\issgpr}{i{\sc ssgpr}\xspace}
\newcommand{\rgls}{{\sc rgls}\xspace}
\newcommand{\krgls}{{\sc krgls}\xspace}
\newcommand{\lwr}{{\sc lwr}\xspace}
\newcommand{\lwpls}{{\sc lwpls}\xspace}
\newcommand{\lgpr}{{\sc lgp}\xspace}
\newcommand{\nusvr}{$\nu$-{\sc svr}\xspace}
\newcommand{\losvr}{{\sc l}o{\sc svr}\xspace}
\newcommand{\svr}{{\sc svr}\xspace}
\newcommand{\svm}{{\sc svm}\xspace}
\newcommand{\svms}{{\sc svm}s\xspace}
\newcommand{\lssvm}{{\sc ls-svm}\xspace}
\newcommand{\sogp}{{\sc sogp}\xspace}
\newcommand{\rfwr}{{\sc rfwr}\xspace}
\newcommand{\soms}{{\sc som}s\xspace}
\newcommand{\som}{{\sc som}\xspace}
\newcommand{\gpr}{{\sc gpr}\xspace}
\newcommand{\ema}{{\sc em}\xspace}
\newcommand{\ofl}{off-line\xspace}
\newcommand{\onl}{on-line\xspace}
\newcommand{\Ofl}{Off-line\xspace}
\newcommand{\Onl}{On-line\xspace}
\newcommand{\ofp}{off-policy\xspace}
\newcommand{\onp}{on-policy\xspace}
\newcommand{\td}{temporal difference\xspace}
\newcommand{\epse}{episodic policy search\xspace}
\newcommand{\epsa}{episodic-sample\xspace}
\newcommand{\epsas}{episodic-samples\xspace}
\newcommand{\ssa}{step-sample\xspace}
\newcommand{\rwa}{reward-weighted averaging\xspace}
\newcommand{\ssas}{step-samples\xspace}
\newcommand{\edas}{{\sc EDA}s\xspace}
\newcommand{\pse}{policy search\xspace}
\newcommand{\Pse}{Policy search\xspace}
\newcommand{\ngo}{natural gradient optimization\xspace}
\newcommand{\Ngo}{Natural gradient optimization\xspace}
\newcommand{\vgo}{vanilla gradient optimization\xspace}
\newcommand{\Vgo}{Vanilla gradient optimization\xspace}
\newcommand{\pid}{$\mathcal{PID}$\xspace}
\newcommand{\pd}{$\mathcal{PD}$\xspace}
\newcommand{\sqp}{{\sc sqp}\xspace}
\newcommand{\gep}{{\sc gep}\xspace}
\newcommand{\geps}{{\sc gep}s\xspace}
\newcommand{\qp}{{\sc qp}\xspace}
\newcommand{\sgn}{{\sc s-gn}\xspace}
\newcommand{\sint}{{\sc s-in}\xspace}
\newcommand{\srn}{{\sc s-rn}\xspace}
\newcommand{\sds}{{\sc s-ds}\xspace}
\newcommand{\sflat}{{\sc s-flat}\xspace}
\newcommand{\cgn}{{\sc c-gn}\xspace}
\newcommand{\cint}{{\sc c-in}\xspace}
\newcommand{\crn}{{\sc c-rn}\xspace}
\newcommand{\cds}{{\sc c-ds}\xspace}
\newcommand{\cflat}{{\sc c-flat}\xspace}
\newcommand{\gn}{{\sc gn}\xspace}
\newcommand{\inter}{{\sc in}\xspace}
\newcommand{\rnet}{{\sc rn}\xspace}
\newcommand{\ds}{{\sc ds}\xspace}
\newcommand{\flt}{{\sc flat}\xspace}
\newcommand{\ai}{{\sc ai}\xspace}
\newcommand{\acl}{{\sc acl}\xspace}
\newcommand{\roll}{rollout\xspace} % discount factor
\newcommand{\rolls}{rollouts\xspace} % discount factor

\newcommand{\robotcub}{{\sc RobotCub}\xspace}
\newcommand{\atr}{{\sc atr}\xspace}
\newcommand{\sarsa}{{\sc Sarsa}\xspace}
\newcommand{\ql}{{\sc q-learning}\xspace}
\newcommand{\barrett}{{\sc Barrett}\xspace}
\newcommand{\icub}{{\sc iCub}\xspace}
\newcommand{\james}{{\sc James}\xspace}

\newcommand{\mymath}[1]{\ensuremath{#1}\xspace}
\newcommand{\mymathbf}[1]{\mymath{\mathbf{\boldsymbol{#1}}}}
\newcommand{\covar}{\mymathbf{\Sigma}}
\newcommand{\vtheta}{\mymathbf{\theta}}

\renewcommand{\vec}[1]{\mymathbf{#1}}
\newcommand{\mat}[1]{\mymathbf{#1}}
%\newcommand{\eps}{\vec{\epsilon}}

\newcommand{\varinit}{\mymath{\covar^{\mbox{\scriptsize init}}}}

\newcommand{\mX}{\mat{X}}
\newcommand{\mG}{\mat{G}}
\newcommand{\mF}{\mat{F}}
\newcommand{\vomega}{\vec{\omega}}
\newcommand{\Vomega}{\vec{\Omega}}
\newcommand{\vs}{\vec{s}}
\newcommand{\vo}{\vec{o}}
\newcommand{\vu}{\vec{u}}
\newcommand{\vx}{\vec{x}}
\newcommand{\vw}{\vec{w}}
\newcommand{\vj}{\vec{j}}
\newcommand{\vphi}{\vec{\phi}}
\newcommand{\VO}{\mathcal{O}}
\newcommand{\U}{\mathcal{U}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\E}{\mathcal{E}}
\newcommand{\T}{\mathcal{T}}

\newcommand{\f}{\mymath{f}}
\newcommand{\inpu}{\vec{\phi}}
\newcommand{\Inpu}{\mymath{\Phi}}
\newcommand{\vinpu}{\mymath{\tilde{\vec{\phi}}}}
\newcommand{\Vinpu}{\mymath{\tilde{\Phi}}}
\newcommand{\vnabla}{\mymath{\tilde{\nabla}_{\vinpu}}}
\newcommand{\vf}{\mymath{\tilde{\f}}}

\newcommand{\hatf}{\mymath{\hat{\f}}}
\newcommand{\hatj}{\mymath{\hat{J}}}
\newcommand{\hatq}{\mymath{\hat{Q}}}
\newcommand{\hatv}{\mymath{\hat{V}}}
\newcommand{\hatu}{\mymath{\hat{U}}}

\newcommand{\her}{{\sc her}\xspace}
\newcommand{\mcher}{{\sc mc-her}\xspace}
\newcommand{\gcp}{{\sc gcp}\xspace}
\newcommand{\gcps}{{\sc gcp}s\xspace}
\newcommand{\uvfa}{\textsc{uvfa}\xspace}
\newcommand{\uvfas}{{\sc uvfa}s\xspace}
\newcommand{\mtl}{{\sc mtl}\xspace}
\newcommand{\mrl}{{\sc mrl}\xspace}
\newcommand{\hrl}{{\sc hrl}\xspace}
\newcommand{\maml}{{\sc maml}\xspace}
\newcommand{\fomaml}{{\sc fomaml}\xspace}
\newcommand{\reptile}{{\sc reptile}\xspace}
\newcommand{\pearl}{{\sc pearl}\xspace}
\newcommand{\maesn}{{\sc maesn}\xspace}
\newcommand{\fr}{{\sc FetchReach}-v1\xspace}
\newcommand{\fp}{{\sc FetchPush}-v1\xspace}
\newcommand{\fs}{{\sc FetchSlide}-v1\xspace}
\newcommand{\fpap}{{\sc FetchPickAndPlace}-v1\xspace}
\newcommand{\fetch}{{\sc Fetch}\xspace}

\newcommand{\imgep}{\textsc{imgep}\xspace}
\newcommand{\fun}{{\sc f}u{\sc n}\xspace}
\newcommand{\darla}{{\sc darla}\xspace}
\newcommand{\distral}{{\sc distral}\xspace}
\newcommand{\unicorn}{{\sc unicorn}\xspace}
\newcommand{\saggriac}{{\sc sagg-riac}\xspace}
\newcommand{\iac}{{\sc iac}\xspace}
\newcommand{\ggan}{Goal{\sc gan}s\xspace}
\newcommand{\ogan}{Option{\sc gan}s\xspace}
\newcommand{\hdqn}{h-{\sc dqn}\xspace}
\newcommand{\hiro}{{\sc hiro}\xspace}
\newcommand{\asap}{{\sc asap}\xspace}
\newcommand{\rig}{{\sc rig}\xspace}
\newcommand{\hierq}{{\sc hierq}\xspace}
\newcommand{\hac}{{\sc hac}\xspace}
\newcommand{\hacob}{{\sc hacob}\xspace}
\newcommand{\ugl}{{\sc ugl}\xspace}
\newcommand{\mugl}{{\sc mugl}\xspace}
\newcommand{\diayn}{{\sc diayn}\xspace}
\newcommand{\discern}{{\sc discern}\xspace}
\newcommand{\curious}{{\sc curious}\xspace}
\newcommand{\imagine}{{\sc imagine}\xspace}
\newcommand{\lgb}{{\sc lgb}\xspace}
\newcommand{\decstr}{{\sc decstr}\xspace}
\newcommand{\zpd}{{\sc zpd}\xspace}
\newcommand{\socialp}{{\sc sp}\xspace}
\newcommand{\gangstr}{{\sc gangstr}\xspace}
\newcommand{\clic}{{\sc clic}\xspace}
\newcommand{\vic}{{\sc vic}\xspace}

\newcommand{\mt}{multitask\xspace}
\newcommand{\Mt}{Multitask\xspace}

\newcommand{\cs}{{\sc c}s\xspace}
\newcommand{\competence}{{\sc c}\xspace}
\newcommand{\lp}{{\sc lp}\xspace}
\newcommand{\proba}{{\sc p}\xspace}

\newcommand{\mujoco}{{\sc mujoco}\xspace}

\newcommand\wi[1]{$\circ$}
\newcommand\bu[1]{$\bullet$}
\newcommand\ot[1]{$\star$}
\newcommand\spa[1]{$\spadesuit$}
\newcommand\dn[1]{.}
\newcommand\no[1]{}
\newcommand\bo[1]{$\bullet\star$}

\usepackage{array}

\newcommand\partielle[2]{\frac{\partial #1}{\partial #2}} % partial derivative

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=1pt] (char) {\tiny #1};}}

\newcommand{\fk}{{$\mathcal{FK}$}\xspace}

%%% MDP and RL specific commands
\newcommand\pol{\pi} % policy
\newcommand\Pol{\Pi} % policy-space
\newcommand{\params}{{\mymathbf{\theta}}\xspace} % policy parameters (vector)
\newcommand{\Params}{\mymath{\Theta}}
\newcommand{\disc}{\gamma} % discount factor

\newenvironment{definition}{{\bf Definition:}}{\par}
\newenvironment{property}{{\bf Property:}}{\par}
\newenvironment{remark}{{\bf Remark:}}{\par}
\newenvironment{example}{{\bf Example:}}{\par}

\newcounter{cbox} \setcounter{cbox}{0}
\newcommand{\cbox}{\arabic{cbox}}
\newenvironment{mybox}[2]{\refstepcounter{cbox}\begin{tcolorbox}[title=Box \cbox: #1]\label{#2}\par}{\end{tcolorbox}}

\newcounter{cmes} \setcounter{cmes}{0}
\newcommand{\cmes}{\arabic{cmes}}
\newenvironment{mymes}[1]{\begin{tcolorbox}[colback=red!10!white]\refstepcounter{cmes}{\bf Message \cmes:}\label{#1}}{\end{tcolorbox}}

\usepackage{xcolor}
\definecolor{myred}{rgb}{0.8,0,0}
\definecolor{mypurple}{rgb}{0.6,0.22,0.8}

\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{myblue}{rgb}{0,0,0.7}
\definecolor{myindigo}{rgb}{0.4,0,0.7}
\newcommand{\new}[1]{\textcolor{myblue}{\fbox{\bf New:}{\em #1}}}
\newcommand{\note}[1]{\textcolor{myindigo}{\fbox{\bf Note: {\em #1}}}}
\newcommand{\biblio}[1]{\textcolor{myblue}{\fbox{\bf Todo:}{\em #1}}}
\newcommand{\todolater}[1]{\textcolor{myblue}{\fbox{\bf Todo:}{\em #1}}}
\newcommand{\todiscuss}[1]{\textcolor{mygreen}{\fbox{\bf To discuss:}{\em #1}}}

\newcommand{\todo}[1]{\textcolor{myred}{\fbox{\bf Todo:}{\em #1}}}
\newcommand{\ahmed}[1]{\textcolor{mypurple}{\fbox{\bf Ahmed:}{#1}}}
\newcommand{\os}[1]{\textcolor{mygreen}{\fbox{\bf Olivier:}{\em #1}}}
\newcommand{\mohamed}[1]{\textcolor{myred}{\fbox{\bf Mohamed:}{\em #1}}}
\newcommand{\hugo}[1]{\textcolor{myblue}{\fbox{\bf CC:}{\em #1}}}


% \newcommand{\comments}[1]{}
% \newcommand{\todo}[1]{\comments{#1}}
% \newcommand{\ahmed}[1]{\comments{#1}}
% \newcommand{\os}[1]{\comments{#1}}
% \newcommand{\mohamed}[1]{\comments{#1}}
% \newcommand{\cc}[1]{\comments{#1}}

